Evaluation of the Performance/Energy Overhead in DSP Video Decoding and its Implications

Video decoding is considered as one of the most compute and energy intensive application in energy constrained mobile devices. Some specific processing units, such as DSPs, are added to those devices in order to optimize the performance and the energy consumption. However, in DSP video decoding, the inter-processor communication overhead may have a considerable impact on the performance and the energy consumption. In this paper, we propose to evaluate this overhead and analyse its impact on the performance and the energy consumption as compared to the GPP decoding. Our work revealed that the GPP can be the best choice in many cases due to the a significant overhead in DSP decoding which may represents 30% of the total decoding energy.

==> backgroud.tex <==

\section{Backgroud}
\label{backgroud}

As described in the introduction, the performance and energy properties of video decoding depends on the used processing elements (processor type and clock frequency) and on the video coding quality. We describe hereafter how this is reflected at both architecture and system level.

A  video consists of a data stream which is processed sequentially to produce the decoded video. The digital circuit clock frequency partly determines  the decoding time and the power consumption. In fact, in CMOS circuits, the dynamic power consumption is described  by the following equation :
\begin{equation}
\label{DVFS-P-EQUATION}
P_{dyn}=C_{eff}.V^2.f
\end{equation}
where $C_{eff}$ represents the circuit effective capacitance, $V$,   the supply voltage associated to the clock frequency  $f$ \cite{375385}. 

For instance,  Figure \ref{system-arch-vfs} shows a simplified representation of a CMOS circuit which processes a set of data $D$ using a bloc $B$. The bloc $B$  operates at  frequencies $\frac{f}{2}$ (Fig. \ref{system-arch-vfs}-b) and $f$ (Fig. \ref{system-arch-vfs}-a) corresponding to the supply voltage levels  $V_1=1.06V$ and $V_2=1.2V$ respectively\footnote{$V_1$ and $V_2$ are the voltage levels associated to the frequencies 500 Mhz and 250 Mhz of the Cortex A8 processor used in our experimental study.}. If we suppose the processing time is $t$ then the energy consumption when $B$ operates at a frequency $f$ is $E_{V_2}=P_{V_2}.t$ where $P_{V_2}=C_{eff}.V_2^2.f$.  Fig. \ref{system-arch-vfs}-a illustrates this configuration.


Fig. \ref{system-arch-vfs}-b shows the case where $B$ operates at the  frequency $\frac{f}{2}$. If we suppose the processing time at frequency $\frac{f}{2}$ is doubled, then the ratio between the energy $E_{V_1}$ consumed  by the circuit at the frequency $\frac{f}{2}$ with $V_1=1.06V$, and  $E_{V_2}$  is :
\begin{equation*}
\dfrac{E_{V_1}}{E_{V_2}}=\frac{C_{eff}.V_1^2.\frac{f}{2}.2.t}{C_{eff}.V_2^2.f.t}= (\dfrac{V_1}{V_2})^{2} \simeq \frac{4}{5}
\end{equation*}

\begin{figure}[!h]
\centering
\includegraphics[width=2.75in]{figs/dvfs-vs-parallelism.pdf}
 \caption{System  and architecture driven frequency scaling}
 \label{system-arch-vfs}
\end{figure}

\noindent In this case,  scaling down the voltage and the frequency decreases  the power consumption to $P_{V_1}=C_{eff}.V_1^2.\frac{f}{2}\simeq \frac{2}{5}.P_{V_2}$ which leads to 20\% energy saving at the cost of performance decrease. This may represent a scenario where the operating system scales-down dynamically the  processor frequency at run time when it detects a load decrease. This illustrates a system-driven voltage scaling.

In order to save energy without sacrificing the performance, an architectural-driven voltage scaling \cite{chandrakasan_low-power_1992} can be achieved by using two $B$ blocks which are both clocked at a frequency $\frac{f}{2}$ and a voltage $V_1$  as described in Fig. \ref{system-arch-vfs}-c. We note the consumed power and energy associated to this configuration  $P_{2.V_1}$ and $E_{2.V_1}$ respectively. Since two blocks are operating in parallel, the execution time is not  deceased and the ratio between $E_{2.V_1}$ and $E_{V_2}$ is :
\begin{equation*}
\dfrac{E_{2.V_1}}{E_{V_1}}=\dfrac{C_{eff}.V_1^2.\frac{f}{2}.t+C_{eff}.V_1^2.\frac{f}{2}.t}{C_{eff}.V_2^2.f.t}=(\dfrac{V_1}{V_2})^{2}\simeq \frac{4}{5}
\end{equation*}
  
\noindent In this configuration, the total power consumption $P_{2.V_1}$ is the sum of the power consumptions of the two blocks $2.C_{eff}.V_1^2.\frac{f}{2}=\frac{4}{5}.P_{V_2}$ and the energy saving is equal to 20\% without sacrificing the performance but at a cost of an additional circuit area. Theoretically, this type of parallelism provides better performance and energy efficiency for multimedia data processing applications  \cite{chandrakasan_low-power_1992}. However, it generates an energy overhead in both architectural level and system level. In fact, the duplication of the processing circuits and the use of multiplexing/demultiplexing circuits in the architecture consumes more leakage energy \cite{1317052}.

When this type of parallel architecture is implemented in an additional specialized processors such as DSPs \footnote{Parallelism can be used internally in GPPs using pipeline and SIMD instructions.}, the GPP-DSP inter-processor communication may generate a system overhead, and thus yet another additional energy consumption \cite{DSP-overhead-article, CodecEngineOverhead}. As an illustration, Fig. \ref{DSP-video-decoding} describes the steps of a typical DSP video decoding process controlled by a GPP : 
\label{dsp-overhead}

\begin{figure}[!h]
\centering
\includegraphics[width=3in]{figs/dsp-decoding.pdf}
 \caption{DSP video decoding}
 \label{DSP-video-decoding}
\end{figure}

\begin{enumerate}

\item The GPP writes-back the frame located in its cache to a shared memory so that the DSP can access it.
\item The GPP sends the parameters to the DSP codec via a GPP-DSP hardware bus.
\item The DSP cache invalidates the entries in its cache corresponding to a frame buffer in the shared memory.
\item The DSP decodes and transfers the frame to the output buffer.
\item The DSP sends the return status to the GPP.  

\end{enumerate}

\noindent The fact that both the DSP and the GPP have their proper cache memory and communicate using a shared memory imposes to manage cache coherency each time the DSP shares a data with the GPP. In addition, from the operating system level, The GPP-DSP communication is managed by a driver through a system call. A frame decoding is considered, from the GPP point of view, as an I/O operation generating a system latency caused by entering the \textit{idle} state and handling of hardware interrupt. 

So, in order to fully compare GPP and DSP performance for video decoding, one must pay a particular attention to the additional communication overhead when choosing the DSP processing element and not only compare raw performances of both processors.
%In what follows, we consider the evaluation of system overhead in case of DSP video decoding and what is its impact on the performance as compared to a GPP video decoding in case of using different clock frequencies and video coding qualities. 


	


==> conclusion.tex <==

\section{Conclusion}
\label{Conclusion}



The obtained experimental results revealed that the best performance-energy trade-off highly depends on the required video bit-rate and resolution as the GPP can be the best choice in many cases. In fact, the characterization achieved in this work showed that in case of low video bit-rate and resolution, the  DSP decoding suffers from a considerable inter-processor overhead leading to a degradation in the performance and energy efficiency.   



In this paper, we realized a comprehensive study of the performance and the energy consumption of ARM and DSP H264/AVC video decoding. A system and application level characterization methodology was proposed to evaluate the performance and energy proprieties of the H264/AVC GPP and DSP decoding in terms of architecture, system and application parameters. 

An important contribution of our work is the evaluation of the performance and energy overhead of GPP and DSP video decoding for different video bit-rates and resolution. It was shown that in case of low video coding qualities, the system overhead represents an important part in the case of DSP decoding  which leads to a degradation in the performance and  energy properties.

The overhead evaluation results was used to explain the overall performance and   energy properties of both GPP and DSP video decoding. This allowed to define the video coding qualities where using a GPP is more energy efficient than using a DSP. The results are based on an experimental tests conducted on OMAP3530 low-power platform, however, our methodology can be applied on any other platform for  performance and energy evaluation.

The result of this work can be used as a guidelines for selecting the appropriate processing element of the studied \textit{SoC} when decoding a video having a given video bit-rate and resolution. An interesting application (we plan to implant) is to use these guidelines to select dynamically the processor type to be used in an energy-ware decoding for dynamic streaming \cite{Stockhammer:2011:DAS:1943552.1943572, schwarz_overview_2007}  where the quality of the decoded video change dynamically according the the bandwidth fluctuation or the mobile device displaying capabilities.

  

\section*{Acknowledgment}



==> gdr2013.tex <==
\begin{abstract}
%\boldmath

Mobile devices such as smart-phones and tablets are increasingly becoming the most important channel for delivering end-user Internet traffic especially multimedia content. One of the most popular use of these terminals is video streaming. In this type of application, video decoding is considered as  the most compute and  energy intensive part. Some specific processing units, such as  DSPs, are added to those devices in order to optimize the performance and energy consumption. However, in DSP video decoding, the inter-processor communication overhead may have an impact on the performance and the energy consumption as compared to the GPPs. In fact, our work revealed that the GPP can be the best choice in many cases due to the a significant overhead in DSP decoding which may represents 30\% of the total decoding energy in some cases.

\begin{IEEEkeywords}
Video decoding, Performance, Energy, GPP, DSP, H264/AVC, OMAP, Gstreamer. 
\end{IEEEkeywords}
   
\end{abstract}
\section{Introduction}


Energy saving consideration becomes at the center of the hardware and the application design in mobile devices such as smart-phones and tablets. In fact, Lithium battery technologies are not evolving fast enough, this negatively impacts  the autonomy duration. This is becoming a critical issue especially when using processor intensive applications such as video playback.  In \cite{carroll2010analysis}, it is shown that video playback is the most important energy consumer application used in mobile devices. This is due to the important use of the processing resources responsible of more than 60\% of the consumed energy \cite{carroll2010analysis}.

Furthermore, to allow high quality video decoding, the processors equipping mobile devices are more and more powerful. A hardware configuration including  a processor clocked at more than 1 GHz frequency becomes common. The main drawback of using high frequencies is that it requires higher voltage levels. This leads to a considerable increase in energy consumption due to the quadratic relation between the dynamic power and the supplied voltage in CMOS circuits. To overcome this issue,  Digital Signal Processors (DSP) are used  to provide better performance-energy properties. Indeed, the use of parallelism in data processing increases the performance without the need to use higher voltages and frequencies \cite{1317052}. 

In case of DSP decoding, in addition, to the clock frequency and the decoded video quality parameters stated above, the  overhead due to the inter-processor communication should  be considered. This issue was addressed from performance point in studies such as \cite{5657208,1598326}. However its impact on the energy consumption as compared to a GPP decoding was not studied before.  In this paper, we propose to evaluate the performance and the energy overhead in DSP decoding and analyse its impact on the performance and the energy consumption as compared to GPP video decoding. For this purpose, we conduct an experimental measurements which are described in section \ref{Experimental setup}. The obtained results and the conclusion are discussed in sections \ref{Results and discussion} and \ref{Conclusion} respectively.

 \section{Experimental Methodology and Setup}


\label{Experimental setup}

\label{experiment-methodology}

\noindent In the experimentations, we followed two steps. 1) A video frame level performance and energy characterization where the DSP  performance and energy overhead is evaluated in a frame decoding cycle. We define the overhead as all the processing witch is not related to the actual frame decoding such as GPP-DPP communication and cache memory maintenance operations. 2) The video sequence performance and energy consumption are evaluated and compared to those of the GPP. 

Power measurements performed in this study were achieved using the Open-PEOPLE framework \cite{sennopenpeople}, a multi-user and multi-target power and energy optimization platform and estimator. The target platform is OMAP3530EVM board which consists of a Cortex A8 ARM processor and TMS320C64x DSP. The  power consumptions of the DSP and the ARM processors are measured using . On this hardware platform, the Linux operating system version 2.6.32 was used. The video decoding was achieved using \textit{Gstreamer}, a multimedia development framework. The ARM decoding, was performed using \textit{ffdec\_h264}, an open-source plug-in based on   \textit{ffmpeg/libavcodec} library. For DSP decoding, we used \textit{TIViddec2}, a proprietary Gstreamer H264/AVC baseline profile plug-in provided by \textit{Texas Instrument}. The videos sequences used in the tests are Harbor and Soccer. Each video is coded in  different biterates (64 Kb/s, \ldots 5120 Kb/s) and \textit{qcif}, \textit{cif} and \textit{4cif} resolutions. Each video is then  decoded at different clock frequencies ranging from 125 MHz to 720 MHz. The performance (Frame/s) and the energy consumption (mJ/frame) are measured for each (bit-rate, resolution, frequency). 

\section{Experimental Results \& Discussions}



\begin{figure*}[!t]
\centering
\includegraphics[width=1.7in]{figs/fps-bitrate-qcif-harbour.pdf}
\includegraphics[width=1.7in]{figs/fps-bitrate-cif-harbour.pdf}
\includegraphics[width=1.7in]{figs/fps-bitrate-4cif-harbour.pdf}
 \caption{ARM and DSP decoding performance of the Harbour video}
\label{3d-fps}
\end{figure*}

\begin{figure*}[!t]
\centering
\includegraphics[width=1.7in]{figs/jpf-bitrate-qcif-harbour.pdf}
\includegraphics[width=1.7in]{figs/jpf-bitrate-cif-harbour.pdf}
\includegraphics[width=1.7in]{figs/jpf-bitrate-4cif-harbour.pdf}

 \caption{ARM vs DSP decoding energy consumption of H264/AVC video}
\label{3d-energy}
\end{figure*}

\label{Results and discussion}

\subsection{Frame level Performance and energy characterization}

Fig. \ref{frame-dec} shows the power consumption level of \textit{4cif} and \textit{qcif} DSP video decoding. The DSP frame decoding phase is represented by the band varying between 0.7 W and 1.1 W corresponding to [32 ms, 62ms] and [6.2 ms, 7.5ms] intervals. This phase  is terminated by a burst of DMA transfers of the decoded frame macro-blocks from the DSP cache to the shared memory which corresponds to the intervals [56 ms, 62ms] and [7.2 ms, 7.5ms] and is illustrated by an increase in memory power consumption. The ARM wake-up latency is represented  by the power level 0.66 W. The ARM wake-up is represented by the power transition to 0.83 W. Table \ref{table-time-overhead} shows the obtained time and energy overhead values for \textit{qcif}, \textit{cif} and \textit{4cif} videos. One can notices that the time and energy overhead can reach 50\% and 30\% respectively  in case of \textit{qcif} resolution. 
\label{frame-characterization}
\begin{figure}[!h]	
\centering
\includegraphics[width=1.7in]{figs/4cif-dsp.pdf}
\includegraphics[width=1.7in]{figs/qcif-dsp.pdf}
\caption{ARM and DSP frames decoding}
\label{frame-dec}
\end{figure}

\begin{table}[h]
\caption{\small {DSP video decoding time and energy overhead}}
\label{table-time-overhead}

\scalebox{0.83}
{
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline 
\multirow{2}{*}{Resolution} & \multicolumn{3}{c|}{DSP decoding energy(mJ/frame)} & \multicolumn{3}{c|}{DSP decoding time (ms/frame)}\tabularnewline
\cline{2-7} 
 & Processing  & Total  & Overhead (\%) & Processing  & Total  & Overhead (\%)\tabularnewline
\hline 
qcif (128kb) & 1.97 & 4.16 & 52.64 & 1.71 & 2.33 & 30.48\tabularnewline
\hline 
cif (1024kb) & 6.016 & 8.36 & 28.11  & 5.35 & 6.72 & 20.38\tabularnewline
\hline 
4cif (5120 kb) & 23.73 & 25.93 & 8.48 & 21.59 & 22.16 & 2.5\tabularnewline
\hline 
\end{tabular}
}
\end{table}


\subsection{Video Stream Performance and Energy Evaluation}

\subsubsection{Decoding Performance Results}
\label{performance}

Fig. \ref{3d-fps} shows a comparison between ARM and DSP video decoding performance in case of \textit{4cif}, \textit{cif} and \textit{qcif} resolutions for the Harbor video sequence. The flat surface represents the reference video displaying rate (30 Frames/s). One can notes that the performances of the ARM processor and of the DSP are almost equivalent in case of \textit{qcif} resolution. However, the ARM decoding speed is 43\% higher than the DSP in case of 64 Kb/s bit-rate while the DSP decoding speed is 14\%  higher than the ARM in case of 5120 Kb/s bit-rate.  For \textit{cif} and \textit{4cif} resolutions, The DSP decoding is almost 50 \% faster than of the ARM in case of \textit{cif} resolution and 100\% in case of \textit{4cif}. This ratio decreases drastically  for low bit-rates where the ARM performance  increases faster than the one of the DSP.


\subsubsection{Energy Consumption Results}

Fig. \ref{3d-energy} shows a comparison between  the ARM and DSP video decoding  energy consumption (mJ/Frame) in case of \textit{4cif}, \textit{cif} and \textit{qcif} resolutions. The DSP \textit{qcif} video decoding consumes 100\% more energy than the ARM in case of low bit-rate and 20\% for high bit-rate.  On the other hand, the DSP \textit{4cif} video decoding consumes less energy than the ARM although.  In case of  \textit{cif} resolution, we  noticed an crossing between the ARM and the DSP energy consumption levels. In fact, for low bit-rate starting from 1Kb/s, the ARM consumes less energy than the DSP.

\section{Conclusion}
\label{Conclusion}

The analysis of the results shows that the overall performance and the energy efficiency of the DSP as compared to the ARM processor depend mainly on the required video coding quality (Bit-rate and resolution). In fact, the DSP video decoding is the best performance and energy efficient choice  in case of \textit{4cif} resolution and the use of ARM decoding is better in case of \textit{qcif} resolution and  \textit{cif} resolution with a bit-rate less than 1 Mb/s. The deterioration of the performance and energy consumption properties of the DSP video decoding are due to a significant inter-processors overhead. 

==> methodology.tex <==
\section{Performance and Energy Characterization Methodology}
\label{Methodology}

In this work, we chose to characterize H264/AVC  \cite{wiegand_overview_2003} video decoding standard.  Although other solutions are emerging, such as HEVC \cite{hevc} and VP8 \cite{vp8}, H264/AVC stays the most mature used standard.

An H.264/AVC video consists of a sequence of frames (Coded Pictures). Each frame may depend on previous and/or next frames and its decoding requires the execution of different steps  such as entropy decoding, inverse transform, motion compensation \cite{wiegand_overview_2003}. Each step is characterized by its performance and energy consumption properties \cite{macomplexity2011} which highly depend on the underlying execution platform \cite{1218201}. In our methodology, we decided to characterize the performance and the energy consumption of video decoding regardless of the internal intricacies of H.264/AVC decoding process. For this purpose, we propose a performance characterization methodology which intervenes at three hierarchical levels : 

\begin{figure}[!t]
\centering
\includegraphics[width=1.7in]{figs/methodology2.pdf}
 \caption{Performance and energy characterization levels}
 \label{fig-methodology}
\end{figure}

\begin{enumerate}
\newdimen\origiwspc%
\origiwspc=\fontdimen2\font
%\fontdimen2\font=0.2ex% inter word space

\item Operating system level.
\item Video frame level.
\item Video sequence level.
%\fontdimen2\
\fontdimen2\font=\origiwspc
\end{enumerate}

\noindent As depicted in Fig. \ref{fig-methodology}, the results of each level serves to characterize and understand the performance and the energy properties of upper level. In what follows, each level is described.

\subsection{Operating System Level Power Characterization}

In this step, the power consumption of both the GPP and the DSP at the \textit{idle} and the active states are measured at different clock frequencies regardless of any video decoding process. The objective of this level is to constitute a set of reference power consumption values that help to understand and quantify the performance and the energy consumption of the different video decoding process phases at a frame granularity.

\subsection{Frame-level Performance and Energy Characterization}

This is the most important step, in our methodology, that helps to understand the global performance study. It is related to  both operating system and decoder application. At this level, the elementary video frame decoding is characterized in terms of a set of parameters such as buffer transfers, GPP-DSP communication and cache coherency maintenance. The objective of this step is to understand how the processing elements are used and where goes the energy when decoding a single frame. As discussed farther, in this step, we evaluated the overhead of both GPP and DSP video decoding process. This level relies on the preceding operating system level characterization to identify the active and idle processor states.

\label{overhead-definition}

In this level, a frame decoding step includes decoding a given frame located in the memory (in the input buffer) and copying it to the output buffer.  In case of GPP decoding, the overhead is all the application logic controlling the sequential calls to the frame processing functions. In this case, the frame decoding function is local (to the GPP) and the overhead is related to the design of the application decoder. For example, a multi-threaded decoder may induce an overhead due to thread synchronization. We note this kind of overhead as a GPP-overhead.  

On the other hand, in the case of DSP decoding, the frame decoding function is executed in a remote processor (the DSP). As described in section \ref{backgroud}, this induces an overhead due to GPP-DSP communication such as cache maintenance and hardware interrupt handling. We note this kind of overhead a DSP-overhead.  

Both of these different kinds of overheads induce an extra performance and energy costs. We describe in the experimental methodology how these costs have been calculated.


\subsection{Video Sequence Decoding Performance and Energy Characterization}

In this step,  the average performance (number of decoded frames per seconded) of H264/AVC decoding of the overall video sequence is measured in terms of bit-rate, resolution and clock frequency. Both of the GPP and the DSP have been tested. The  chosen performance evaluation criteria was the video displaying rate of the decoded video. In fact we considered that a decoding rate which is lower than the displaying rate of the coded video as not sufficient for playing-back the video with  respect to real time constraints.

The overall energy consumption is then calculated by multiplying the sum of the elementary measured power values by the decoding time. The average energy per frame (mJ/frame) is then obtained by dividing the overall energy on the total frames number.

==> related-works.tex <==
\section{Related Works}


H.264/AVC Video decoding performance and energy consumption characterization issue may be addressed at application, system or architectural levels.


 In \cite{1317052}, the performance and energy consideration when using pipelines and parallelism in CMOS circuits is studied and it was shown why these architectures increase the energy efficiency. In \cite{H264-ASIC}, the particular case of H.264 video decoding is analyzed and an energy-aware processor architecture design methodology is proposed for energy efficient H264/AVC decoding. At this level, the impact on the energy consumption of application and operating system layers are not considered. 
   
At a higher level, In \cite{1218201}, H264/AVC decoding performance is characterized on different GPP processor architectures  at CPU cycle level. This approach is used  in \cite{macomplexity2011} for energy characterization and modeling of the different H264/AVC decoder modules. The results were used to develop an energy-aware video decoding strategy for ARM processor supporting DVFS feature. The result of this study are generalized in  \cite{limodeling2012} for considering the variation in video bit-rate. These studies was focusing only on GPP processor. 

On the other hand, many works studied the performance and energy consumption of DSP video decoding. In \cite{5657208,1598326,DSP-overhead}, performance consideration of DSP decoding are analyzed especially regarding cache coherency maintenance and DMA transfers. In \cite{Julien}, energy characterization of DSP processing is addressed in terms of memory access and DMA transfers. In \cite{juarez_distortion-energy_2012}, DSP video decoding energy consumption is analyzed in terms of different video coding qualities.  Many of these studies highlight the performance and the energy efficiency of the DSP video decoding however, they don't compare them to the performance of GPP video decoding.


In this study, we have proposed to characterize the performance and energy consumption of GPP and DSP H264/AVC video decoding in terms of bit-rate, resolution and clock frequency. To allow an objective evaluation of the GPP decoding as compared to that of the DSP, we focus in the proposed methodology on executing the GPPs and DSPs video decoding performance and energy measurement under the same condition by using a \textit{Gstreamer} a GPP-DSP mutimedia framework.  As far as we know, no study considered all these parameters for both GPP and DSP  within the same application framework. 

\label{Related Works}

